Testing Updated Apps by Adapting Learned Models

Although App updates are frequent and software engineers would like to verify updated features only, automated testing techniques verify entire Apps and are thus wasting resources. We present Continuous Adaptation of Learned Models (CALM), an automated App testing approach that efficiently test App updates by adapting App models learned when automatically testing previous App versions. CALM focuses on functional testing. Since functional correctness can be mainly verified through the visual inspection of App screens, CALM minimizes the number of App screens to be visualized by software testers while maximizing the percentage of updated methods and instructions exercised. Our empirical evaluation shows that CALM exercises a significantly higher proportion of updated methods and instructions than six state-of-the-art approaches, for the same maximum number of App screens to be visually inspected. Further, in common update scenarios, where only a small fraction of methods are updated, CALM is even quicker to outperform all competing approaches in a more significant way.

==> RQ2plots.tex <==
% !TEX root =  MAIN.tex

\begin{figure*}
\begin{minipage}{.45\textwidth}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_1Hour_COMPARISON_modifiedMethodCoverage}
	\vspace{-1cm}
      \caption{Percentage of updated methods covered for each version of the case studies (budget=1 hour).}
      \label{fig:RQ1:Method:1}
\end{minipage}\hspace{5mm}
\begin{minipage}{.45\textwidth}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_5Hours_COMPARISON_modifiedMethodCoverage}
		\vspace{-1cm}
      \caption{Percentage of updated methods covered for each version of the case studies (budget=5 hours).}
      \label{fig:RQ1:Method:5}
\end{minipage}
\begin{minipage}{.45\textwidth}
	\vspace{-7mm}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_1Hour_COMPARISON_modifiedInstructionsCoverage}
		\vspace{-1cm}
      \caption{Percentage of instructions belonging to updated methods that are covered for each version of the case studies (budget=1 hour).}
      \label{fig:RQ1:Instr:1}
\end{minipage}\hspace{5mm}
\begin{minipage}{.45\textwidth}
	\vspace{-7mm}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_5Hours_COMPARISON_modifiedInstructionsCoverage}
		\vspace{-1cm}
      \caption{Percentage of instructions belonging to updated methods that are covered for each version of the case studies (budget=5 hours).}
      \label{fig:RQ1:Instr:5}
\end{minipage}
\end{figure*}


==> algos/executeTesting.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
\begin{algorithm}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
%\Require \emph{MR}, the bytecode of the metamorphic relation to be executed
%\Require \emph{dataProvider}, an object that exposes the data collected by the crawlers
%\Ensure \emph{Failures}, a list of failing executions with contextual information
% (source inputs, follow-up inputs, output data).

\While { ( NOT stagnation() ) AND ( NOT phaseBudgetConsumed( \emph{phaseBudget}) ) AND (NOT coverageTargetsExercised() ) } \label{algo:test:loop}
	\If { target not selected OR target already exercised OR \emph{visitBudget} exhausted}	\label{algo:test:checkSelectedTarget}
		\State selectTarget() \label{algo:test:select}
		\State identifyPathToTarget() \label{algo:test:path}
	\ElsIf { target unreachable}	\label{algo:test:target:unreachable}
		\State identifyPathToTarget() \label{algo:test:unreachable:path}
	\EndIf


	
\If { NOT\ targetReached() }   \label{algo:test:notTarget}

		\State reachTargetNode( \emph{reachabilityBudget} ) \label{algo:test:reachTarget}
\Else	\label{algo:test:TargetReached}
%	\If { first time the active window is visited }	
%		\State performRandomScrolling()  \label{algo:test:randomScolling}
%	\EndIf	
	\State exerciseTarget( \emph{targetBudget} )	\label{algo:test:execTarget}
\EndIf

	\If {additional random exploration required }   \label{algo:test:randomRequired}
		\State performRandomExploration( \emph{randomExplorationBudget} )	\label{algo:test:execRandom}
	\EndIf
	
\EndWhile



\end{algorithmic}

\caption{\APPR testing algorithm.}
%\vspace{-0.2cm}
\label{alg:testing}
\end{algorithm}



==> algos/generateUpdatedAppModel.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
\begin{algorithm}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
\Require \emph{$M_b$}, the base App Model
\Require \emph{$MW_u$}, the EWTG of the updated version, generated by an extension of Gator
\Require \emph{Diff}, the EWTGDiff computed in the step

%\Require \emph{dataProvider}, an object that exposes the data collected by the crawlers
%\Ensure \emph{Failures}, a list of failing executions with contextual information
% (source inputs, follow-up inputs, output data).
%Fabrizio: since we do not have. a formal definition of the structure of Diff, it is better to have an informal descriptio, same for theothers
\For {each diff $\in$ Window differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markWindowAsAddition(w) \label{algo:genUpdate:markAddition1}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractStates(w) \label{algo:genUpdate:removeAbstractStates}
    \Else
        \State windowReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State reassignAbstractStatesToNewWindow(windowReplacement)
    \EndIf
\EndFor
\For {each diff $\in$ Widget differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markWidgetAsAddition(w) \label{algo:genUpdate:markAddition2}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractValuationMaps(w) \label{algo:genUpdate:removeAVMs}
    \Else
        \State widgetReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State reassignAttributeValuationMapsToNewWidget(widgetReplacement)
    \EndIf
\EndFor
\For {each diff $\in$ Diff$\rightarrow$ Transition differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markTransitionAsAddition(w) \label{algo:genUpdate:markAddition3}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractTransitions(w) \label{algo:genUpdate:removeAbTransitions}
    \Else
        \State transitionReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State t $\gets$ (transitionReplacement$\rightarrow$replaced)
        \State removeAbstractTransitions(t)
    \EndIf
\EndFor
\end{algorithmic}

\caption{\APPR's Updated App model generation}
%\vspace{-0.2cm}
\label{algo:generateUpdatedAppModel}
\end{algorithm}



==> algos/runtimeAdapation.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
\begin{algorithm}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
%\Require \emph{MR}, the bytecode of the metamorphic relation to be executed
%\Require \emph{dataProvider}, an object that exposes the data collected by the crawlers
%\Ensure \emph{Failures}, a list of failing executions with contextual information
% (source inputs, follow-up inputs, output data).
%\While { IsTransitionTriggered() }
\While { waitForTransitionTriggered() }\label{algo:update:loop}
    \State $t$ $\leftarrow$ getRecentAbstractTransition() 
    \State $s_d$ $\leftarrow$ getSourceState($T$)
    \State $s_o$ $\leftarrow$ getResultState($T$)
     \If { IsProcessedBefore($S_O$) } \label{algo:update:observedBefore}
    \State continue
    \EndIf
    \State $S_E$ $\leftarrow$ getExpectedStatesFromBaseModel($T$)
	\For {$s_e$ in $S_E$}
		\If {isObservedState($s_e$)}
			\label{algo:update:stateobservedbefore}
			\State continue
		\EndIf
	    \If { NOT BelongToSameWindow($s_o$,$s_e$)} \label{algo:update:notbelongsamewindow}
	        \State $s_e$ and $s_o$ are nonequivalent \label{algo:update:notbelongsamewindowNE}
	        	\State removeAbstractTransition($s_d$, $s_e$, $t$) \label{algo:update:removeabstracttransition1}
        		\State continue
   	 \EndIf
	 	    \If { isBackwardEquivalent($s_o$, $s_e$) }
        		\State continue
	        \label{algo:update:continuewhenbackequv}
	    \EndIf
   	 \State $s_e$ and $s_o$ are nonequivalent
	    \State removeAbstractTransition($s_d$, $s_e$, $t$) \label{algo:update:removeabstracttransition2}
    \EndFor
\EndWhile
\end{algorithmic}

\caption{\APPR's Runtime adaptation algorithm.}
%\vspace{-0.2cm}
\label{algo:runtimeadaptation}
\end{algorithm}



==> tables/RQ1_VDA_Mannwhitney.tex <==
\begin{table*}[]
\footnotesize
\label{table:RQ1:vda_mannwhitney}
\begin{tabular}{|c|c|c|cccccccc|cccccccc|}
\hline
\multicolumn{1}{|c|}{}             & \textbf{}   & \textbf{}   & \multicolumn{8}{c|}{\textbf{Coverage of target methods}}                                                                                                                                                                                                                        & \multicolumn{8}{c|}{\textbf{Coverage of target instructions}}                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}             & \textbf{}   & \textbf{}   & \multicolumn{4}{c|}{\textbf{A12}}                                                                                                        & \multicolumn{4}{c|}{\textbf{p-value}}                                                                                                & \multicolumn{4}{c|}{\textbf{A12}}                                                                                                        & \multicolumn{4}{c|}{\textbf{p-value}}                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{App}} & \textbf{V1} & \textbf{V2} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AU}} & \multicolumn{1}{c|}{\textbf{M}} & \multicolumn{1}{c|}{\textbf{AT}}     & \multicolumn{1}{c|}{\textbf{AP}}     & \multicolumn{1}{c|}{\textbf{AU}}     & \textbf{M}      & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AU}} & \multicolumn{1}{c|}{\textbf{M}} & \multicolumn{1}{c|}{\textbf{AT}}     & \multicolumn{1}{c|}{\textbf{AP}}     & \multicolumn{1}{c|}{\textbf{AU}}     & \textbf{M}      \\ \hline
activitydiary                      & 105         & 111         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.07}        & \multicolumn{1}{c|}{0.03}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 111         & 115         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.65}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.07}            & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 115         & 118         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 118         & 122         & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 122         & 125         & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.95}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{0.12}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 125         & 130         & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 130         & 131         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.40}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & 0.07            & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \textless{}0.05 \\ \hline
activitydiary                      & 131         & 134         & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 11          & 12          & \multicolumn{1}{c|}{0.89}        & \multicolumn{1}{c|}{0.12}        & \multicolumn{1}{c|}{0.89}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.90}        & \multicolumn{1}{c|}{0.12}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 12          & 16          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 16          & 17          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.46}        & \multicolumn{1}{c|}{0.61}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.16}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.46}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.98}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 16          & 17          & \multicolumn{1}{c|}{0.73}        & \multicolumn{1}{c|}{0.27}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.81}        & \multicolumn{1}{c|}{0.27}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 17          & 18          & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{0.26}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.88}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.26}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 18          & 19          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.99}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.08}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.69}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.08}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            \\ \hline
bbc                                & 19          & 20          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.99}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.52}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
bbc                                & 20          & 21          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.13}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.13}        & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            \\ \hline
bbc                                & 21          & 22          & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.20}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.73}       & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.20}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.73}       & \multicolumn{1}{c|}{0.12}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 22          & 24          & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.39}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.37}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.20}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.25            & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.39}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.38}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.20}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.27            \\ \hline
bbc                                & 24          & 25          & \multicolumn{1}{c|}{0.71}        & \multicolumn{1}{c|}{0.06}        & \multicolumn{1}{c|}{0.83}        & \multicolumn{1}{c|}{0.68}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.09            & \multicolumn{1}{c|}{0.64}        & \multicolumn{1}{c|}{0.06}        & \multicolumn{1}{c|}{0.82}        & \multicolumn{1}{c|}{0.67}       & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.10            \\ \hline
bbc                                & 25          & 26          & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.36}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.86}       & \multicolumn{1}{c|}{0.19}            & \multicolumn{1}{c|}{0.10}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{0.36}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{0.17}            & \multicolumn{1}{c|}{0.10}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 91          & 92          & \multicolumn{1}{c|}{0.81}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.91}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.85}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 92          & 93          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.77}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            \\ \hline
citymapper                         & 93          & 94          & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.26}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.17}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 94          & 95          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.28            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.44}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.33            \\ \hline
citymapper                         & 95          & 96          & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.51}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.67}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.10            \\ \hline
citymapper                         & 96          & 97          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.60}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.22            \\ \hline
citymapper                         & 97          & 98          & \multicolumn{1}{c|}{0.77}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.15            & \multicolumn{1}{c|}{0.68}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.46}       & \multicolumn{1}{c|}{0.13}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
citymapper                         & 98          & 99          & \multicolumn{1}{c|}{0.73}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.15}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.70}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.03}       & \multicolumn{1}{c|}{0.06}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 99          & 100         & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.36}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.14            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.42}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.27            \\ \hline
vlc                                & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.01}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.01}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 18          & 19          & \multicolumn{1}{c|}{0.74}        & \multicolumn{1}{c|}{0.34}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.52}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.34}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.93}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 19          & 22          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.71}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.09            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.65}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            \\ \hline
vlc                                & 22          & 23          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.37}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.74}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.15}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.37}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.23}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.15}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 23          & 24          & \multicolumn{1}{c|}{0.69}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.75}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.77}        & \multicolumn{1}{c|}{0.10}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 24          & 25          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.45}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.45}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.40}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & 0.22            \\ \hline
vlc                                & 25          & 26          & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.98}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.25}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.25}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 26          & 27          & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.44}        & \multicolumn{1}{c|}{0.94}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.30}            & \textless{}0.05 & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{0.21}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 15          & 16          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.21}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.21}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 16          & 17          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.11}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.11}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 18          & 19          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.27}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.27}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 19          & 20          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.88}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & \textbf{10} & 11          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.07}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.90}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.07}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 11          & 12          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 12          & 13          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.06            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 13          & 15          & \multicolumn{1}{c|}{0.56}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.20}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \textless{}0.05 & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.09}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 15          & 16          & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
yahooweather                       & 16          & 17          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.63}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.16}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.75}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 17          & 18          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.09}        & \multicolumn{1}{c|}{0.63}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.17}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.09}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 18          & 19          & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.63}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.53}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
yahooweather                       & 19          & 20          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.10}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.00}       & \multicolumn{1}{c|}{0.14}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \textless{}0.05 \\ \hline
\end{tabular}

\textbf{Legend}: Compared with \emph{AT}, ATUA. \emph{AP}, APE, \emph{AU}, APE-U , \emph{M}, Monkey. For cases in that CALM and the compared tool perform the same (i.e., \(0.44 < A_{12} < 0.56\)), we ignore the p-value.
\caption{Statistical significance and effect size for RQ1}
\end{table*}

==> tables/RQ1_mannwhitney.tex <==
\begin{table}[]
\caption{Statistics signification for RQ1}
\label{table:RQ1:mannwhitney}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{p\_value\_M} & \textbf{p\_value\_I} \\ \hline
activitydiary & 105         & 111         & 0.338                & 0.141                \\ \hline
activitydiary & 111         & 115         & 0.259                & 0.259                \\ \hline
activitydiary & 115         & 118         & 0.035                & 0.057                \\ \hline
activitydiary & 118         & 122         & 0.117                & 0.084                \\ \hline
activitydiary & 122         & 125         & 0.134                & 0.040                \\ \hline
activitydiary & 125         & 130         & 0.037                & 0.047                \\ \hline
activitydiary & 130         & 131         & 0.000                & 0.000                \\ \hline
activitydiary & 131         & 134         & 0.019                & 0.014                \\ \hline
amazefile     & 11          & 12          & 0.032                & 0.022                \\ \hline
amazefile     & 12          & 16          & 0.253                & 0.354                \\ \hline
amazefile     & 16          & 17          & 0.339                & 0.005                \\ \hline
amazefile     & 17          & 18          & 0.186                & 0.209                \\ \hline
amazefile     & 18          & 20          & 0.000                & 0.000                \\ \hline
bbc           & 16          & 17          & 0.301                & 0.431                \\ \hline
bbc           & 17          & 18          & 0.326                & 0.465                \\ \hline
bbc           & 18          & 19          & 0.142                & 0.114                \\ \hline
bbc           & 19          & 20          & 0.378                & 0.037                \\ \hline
bbc           & 20          & 21          & 0.343                & 0.343                \\ \hline
bbc           & 21          & 22          & 0.091                & 0.149                \\ \hline
bbc           & 22          & 24          & 0.422                & 0.435                \\ \hline
bbc           & 24          & 25          & 0.003                & 0.007                \\ \hline
bbc           & 25          & 26          & 0.318                & 0.461                \\ \hline
citymapper    & 91          & 92          & 0.394                & 0.477                \\ \hline
citymapper    & 92          & 93          & 0.464                & 0.375                \\ \hline
citymapper    & 93          & 94          & 0.151                & 0.343                \\ \hline
citymapper    & 94          & 95          & 0.055                & 0.074                \\ \hline
citymapper    & 95          & 96          & 0.177                & 0.322                \\ \hline
citymapper    & 96          & 97          & 0.021                & 0.013                \\ \hline
citymapper    & 97          & 98          & 0.147                & 0.102                \\ \hline
citymapper    & 98          & 99          & 0.262                & 0.341                \\ \hline
citymapper    & 99          & 100         & 0.117                & 0.146                \\ \hline
wikipedia     & 10          & 11          & 0.339                & 0.418                \\ \hline
wikipedia     & 11          & 12          & 0.158                & 0.429                \\ \hline
wikipedia     & 12          & 13          & 0.087                & 0.217                \\ \hline
wikipedia     & 13          & 15          & 0.221                & 0.370                \\ \hline
wikipedia     & 15          & 16          & 0.056                & 0.065                \\ \hline
wikipedia     & 16          & 17          & 0.163                & 0.193                \\ \hline
wikipedia     & 17          & 18          & 0.017                & 0.039                \\ \hline
wikipedia     & 18          & 19          & 0.333                & 0.400                \\ \hline
wikipedia     & 19          & 20          & 0.006                & 0.002                \\ \hline
\end{tabular}
\end{table}

==> tables/RQ1_meanByApp_updatedMethods.tex <==
\begin{table}[h]
\label{table:RQ1:meanByApp}
\caption{Average percentage of covered updated methods and their instructions across Apps}
\begin{tabular}{l|l l l l l}
\hline
\textbf{App}  & \textbf{ATUA} & \textbf{CALM} & \textbf{APE} & \textbf{APE-U} & \textbf{Monkey} \\ \hline
activitydiary & 87.74         & 90.02         & 91.72        & 89.01          & 77.28           \\ \hline
amazefile     & 53.10         & 56.93         & 59.99        & 55.40          & 42.68           \\ \hline
bbc           & 58.06         & 62.53         & 67.08        & 54.38          & 58.88           \\ \hline
citymapper    & 46.05         & 56.69         & 29.96        & 29.32          & 50.67           \\ \hline
vlc           & 63.91         & 71.53         & 76.35        & 68.85          & 68.63           \\ \hline
wikipedia     & 53.69         & 67.96         & 71.16        & 59.43          & 60.50           \\ \hline
yahooweather  & 61.26         & 65.08         & 63.71        & 61.41          & 55.43           \\ \hline \hline
             \textbf{Average} & \textbf{61.19}         & \textbf{67.94}         & \textbf{65.29}        & \textbf{59.16}          & \textbf{60.6}            \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{2cm}|p{3cm}|}
\hline
\textbf{Case}&\multicolumn{1}{|c|}{\textbf{Effort Reduction (avg/min/max)}}\\
\textbf{study}&\multicolumn{1}{|c|}{\textbf{wrt DM2}}\\
\hline
\input{data/RQ2_1Hour_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\input{data/RQ2_5Hours_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\end{tabular}
\caption{Effort reduction with respect to other approaches. Top part shows results with budget of one hour, bottom part shows results for five hours.}
\label{table:RQ2}
\end{table}%


==> tables/RQ2_input.tex <==
\begin{table*}[tb]
\caption{Input data for RQ2}
\label{table:RQ2:input}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{AM\%} & \textbf{CM\%} & \textbf{AW\%} & \textbf{DW\%} & \textbf{CW\%} & \textbf{Aw\%} & \textbf{Dw\%} & \textbf{Cw\%} \\ \hline
activitydiary                          & 105                                   & 111                                   & 3.00                                    & 2.40                                    & 0.00                                    & 0.00                                    & 0.00                           & 0.25                           & 7.48                           & 77.81                          \\ \hline
activitydiary                          & 111                                   & 115                                   & 0.00                                    & 0.90                                    & 0.00                                    & 0.00                                    & 0.00                           & 3.13                           & 3.13                           & 61.10                          \\ \hline
activitydiary                          & 115                                   & 118                                   & 0.90                                    & 4.80                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.59                           & 4.77                           & 65.25                          \\ \hline
activitydiary                          & 118                                   & 122                                   & 4.67                                    & 22.00                                   & 26.67                                   & 0.00                                    & 0.00                           & 39.97                          & 1.94                           & 45.63                          \\ \hline
activitydiary                          & 122                                   & 125                                   & 2.51                                    & 6.05                                    & 0.00                                    & 0.00                                    & 0.00                           & 0.17                           & 0.00                           & 49.92                          \\ \hline
activitydiary                          & 125                                   & 130                                   & 0.93                                    & 4.81                                    & 11.76                                   & 0.00                                    & 0.00                           & 33.75                          & 1.57                           & 41.39                          \\ \hline
activitydiary                          & 130                                   & 131                                   & 0.00                                    & 0.19                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.93                           & 1.93                           & 52.41                          \\ \hline
activitydiary                          & 131                                   & 134                                   & 1.67                                    & 6.22                                    & 5.56                                    & 0.00                                    & 0.00                           & 6.52                           & 7.34                           & 65.14                          \\ \hline
amazefile                              & 11                                    & 12                                    & 6.10                                    & 8.30                                    & 0.00                                    & 0.00                                    & 0.00                           & 19.38                          & 5.54                           & 46.15                          \\ \hline
amazefile                              & 12                                    & 16                                    & 2.95                                    & 4.21                                    & 18.18                                   & 9.09                                    & 36.36                          & 27.21                          & 15.35                          & 45.35                          \\ \hline
amazefile                              & 16                                    & 17                                    & 0.15                                    & 0.20                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.39                           & 1.39                           & 59.33                          \\ \hline
amazefile                              & 17                                    & 18                                    & 2.47                                    & 15.41                                   & 9.09                                    & 0.00                                    & 9.09                           & 10.61                          & 17.17                          & 44.70                          \\ \hline
amazefile                              & 18                                    & 20                                    & 0.00                                    & 0.05                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.50                           & 1.50                           & 54.79                          \\ \hline
bbc                                    & 16                                    & 17                                    & 4.13                                    & 3.39                                    & 8.33                                    & 33.33                                   & 0.00                           & 27.17                          & 56.07                          & 1.16                           \\ \hline
bbc                                    & 17                                    & 18                                    & 0.17                                    & 0.14                                    & 0.00                                    & 0.00                                    & 0.00                           & 21.65                          & 21.65                          & 11.34                          \\ \hline
bbc                                    & 18                                    & 19                                    & 0.28                                    & 0.22                                    & 0.00                                    & 0.00                                    & 0.00                           & 33.33                          & 33.33                          & 4.39                           \\ \hline
bbc                                    & 19                                    & 20                                    & 0.19                                    & 0.09                                    & 4.00                                    & 0.00                                    & 0.00                           & 34.48                          & 32.76                          & 5.17                           \\ \hline
bbc                                    & 20                                    & 21                                    & 3.62                                    & 2.48                                    & 13.79                                   & 13.79                                   & 0.00                           & 36.07                          & 39.34                          & 2.46                           \\ \hline
bbc                                    & 21                                    & 22                                    & 0.96                                    & 1.38                                    & 0.00                                    & 0.00                                    & 0.00                           & 33.93                          & 33.93                          & 3.57                           \\ \hline
bbc                                    & 22                                    & 24                                    & 1.30                                    & 3.87                                    & 13.79                                   & 0.00                                    & 0.00                           & 39.84                          & 31.71                          & 3.25                           \\ \hline
bbc                                    & 24                                    & 25                                    & 0.56                                    & 0.20                                    & 0.00                                    & 10.34                                   & 0.00                           & 30.58                          & 35.54                          & 2.48                           \\ \hline
bbc                                    & 25                                    & 26                                    & 0.57                                    & 0.50                                    & 0.00                                    & 7.69                                    & 0.00                           & 32.76                          & 34.48                          & 4.31                           \\ \hline
citymapper                             & 91                                    & 92                                    & 0.27                                    & 0.26                                    & 0.00                                    & 1.39                                    & 0.00                           & 4.61                           & 4.61                           & 19.74                          \\ \hline
citymapper                             & 92                                    & 93                                    & 0.23                                    & 0.16                                    & 0.00                                    & 0.00                                    & 0.00                           & 5.23                           & 5.23                           & 24.18                          \\ \hline
citymapper                             & 93                                    & 94                                    & 0.40                                    & 0.18                                    & 0.00                                    & 7.04                                    & 0.00                           & 5.23                           & 5.88                           & 22.22                          \\ \hline
citymapper                             & 94                                    & 95                                    & 0.53                                    & 0.23                                    & 0.00                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 21.33                          \\ \hline
citymapper                             & 95                                    & 96                                    & 0.62                                    & 0.60                                    & 0.00                                    & 0.00                                    & 0.00                           & 5.26                           & 5.26                           & 23.68                          \\ \hline
citymapper                             & 96                                    & 97                                    & 0.51                                    & 0.26                                    & 1.49                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 20.00                          \\ \hline
citymapper                             & 97                                    & 98                                    & 0.53                                    & 0.20                                    & 0.00                                    & 0.00                                    & 0.00                           & 3.36                           & 3.36                           & 15.44                          \\ \hline
citymapper                             & 98                                    & 99                                    & 0.04                                    & 0.08                                    & 0.00                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 21.33                          \\ \hline
citymapper                             & 99                                    & 100                                   & 0.55                                    & 0.14                                    & 1.47                                    & 2.94                                    & 0.00                           & 6.49                           & 6.49                           & 22.73                          \\ \hline
wikipedia                              & 10                                    & 11                                    & 4.83                                    & 4.15                                    & 6.90                                    & 13.79                                   & 13.79                          & 26.90                          & 23.43                          & 23.27                          \\ \hline
wikipedia                              & 11                                    & 12                                    & 1.91                                    & 1.63                                    & 0.00                                    & 8.00                                    & 8.00                           & 12.95                          & 35.46                          & 19.89                          \\ \hline
wikipedia                              & 12                                    & 13                                    & 0.82                                    & 0.87                                    & 8.00                                    & 4.00                                    & 4.00                           & 31.88                          & 29.11                          & 11.29                          \\ \hline
wikipedia                              & 13                                    & 15                                    & 2.94                                    & 2.43                                    & 17.24                                   & 0.00                                    & 20.69                          & 33.70                          & 29.81                          & 14.07                          \\ \hline
wikipedia                              & 15                                    & 16                                    & 2.10                                    & 1.85                                    & 6.45                                    & 0.00                                    & 9.68                           & 27.34                          & 9.56                           & 34.03                          \\ \hline
wikipedia                              & 16                                    & 17                                    & 5.99                                    & 10.36                                   & 31.11                                   & 6.67                                    & 8.89                           & 59.64                          & 9.13                           & 25.26                          \\ \hline
wikipedia                              & 17                                    & 18                                    & 2.21                                    & 3.93                                    & 10.64                                   & 4.26                                    & 6.38                           & 48.95                          & 24.07                          & 19.32                          \\ \hline
wikipedia                              & 18                                    & 19                                    & 0.00                                    & 0.15                                    & 0.00                                    & 0.00                                    & 2.22                           & 18.01                          & 17.91                          & 36.18                          \\ \hline
wikipedia                              & 19                                    & 20                                    & 0.31                                    & 0.76                                    & 0.00                                    & 0.00                                    & 2.22                           & 10.41                          & 10.24                          & 44.85                          \\ \hline
\end{tabular}

\footnotesize{\textbf{Legend:} AM\%: Added methods, CM\%: Changed methods, AW\%: Added windows, DW\%: Deleted windows, CW\%: Changed windows, Aw\%: Added widgets, Dw\%: Deleted widgets, Cw\%: Changed widgets }
\end{table*}

==> tables/RQ2_predictionResult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{Y\_1}             & \textbf{P\_1}             & \textbf{Y\_2}             & \textbf{P\_2}             \\ \hline
activitydiary & 105         & 111         & 0                         & 0                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
activitydiary & 111         & 115         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
activitydiary & 115         & 118         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 118         & 122         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 122         & 125         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 125         & 130         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 130         & 131         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 131         & 134         & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 11          & 12          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 12          & 16          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 16          & 17          & 0                         & 0                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
amazefile     & 17          & 18          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 18          & 20          & 0                         & 0                         & 0                         & 0                         \\ \hline
bbc           & 16          & 17          & 0                         & 0                         & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 \\ \hline
bbc           & 17          & 18          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & 0                         & 0                         \\ \hline
bbc           & 18          & 19          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 \\ \hline
bbc           & 19          & 20          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 20          & 21          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
bbc           & 21          & 22          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 22          & 24          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & 0                         & 0                         \\ \hline
bbc           & 24          & 25          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 25          & 26          & 1                         & 1                         & 1                         & 1                         \\ \hline
citymapper    & 91          & 92          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 92          & 93          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 93          & 94          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 94          & 95          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 95          & 96          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
citymapper    & 96          & 97          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 97          & 98          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 98          & 99          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
citymapper    & 99          & 100         & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 10          & 11          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 11          & 12          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 12          & 13          & 1                         & 1                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
wikipedia     & 13          & 15          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
wikipedia     & 15          & 16          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 16          & 17          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 17          & 18          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 18          & 19          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 19          & 20          & 0                         & 0                         & 0                         & 0                         \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2_score.tex <==
\begin{table*}[tb]
\caption{Logistic Regression Model score in predicting success of CALM}
\label{table:RQ2:score}
\begin{tabular}{|l|llll|llll|}
\hline
      & \multicolumn{4}{l|}{Success in coverage of target methods}                                              & \multicolumn{4}{l|}{Success in coverage of target instructions}                                \\ \hline
      & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F1-score} & Support & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F1-score} & Support \\ \hline
\ATUA performs better  & \multicolumn{1}{l|}{0.84}      & \multicolumn{1}{l|}{0.90}   & \multicolumn{1}{l|}{0.87}     & 30      & \multicolumn{1}{l|}{0.85}      & \multicolumn{1}{l|}{0.94}   & \multicolumn{1}{l|}{0.89}     & 31      \\ \hline
\APPR performs better & \multicolumn{1}{l|}{0.62}      & \multicolumn{1}{l|}{0.50}   & \multicolumn{1}{l|}{0.56}     & 10      & \multicolumn{1}{l|}{0.67}      & \multicolumn{1}{l|}{0.44}   & \multicolumn{1}{l|}{0.53}     & 9       \\ \hline
Accuracy   & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{0.8}      & 40      & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{0.82}     & 40      \\ \hline
\end{tabular}
\end{table*}

==> tables/abstraction.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|@{}p{7mm}@{}|@{\hspace{1mm}}p{3.7cm}@{\hspace{1mm}}|@{\hspace{1mm}}p{3.1cm}@{\hspace{1mm}}|}
\hline

\textbf{Level}&\textbf{Reducers applied to interactable Widget}&\textbf{Reducers applied to interactable Widget Children}\\
\hline
L1& $R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E},$ $ R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}$&\\
L2& $R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E},$ $ R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}$, \textcolor{blue}{$R_{T}$}&\\
L3& $R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E},$ $ R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}, R_{T}$, \textcolor{blue}{$R_{HC}$}&\\

L4& $R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E}, $ $R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}, R_{T}$ & 
\textcolor{blue}{$R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E}, $} \textcolor{blue}{$R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}$}\\

L5& $R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E},$  $R_{P},  R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}, R_{T}$ & 
$R_{RID}, R_{CN}, R_{CD}, R_{Ch}, R_{E}, $ $R_{P}, R_{S}, R_{I}, R_{C}, R_{LC}, R_{S}$, \textcolor{blue}{$R_{T}$}\\

\hline

\end{tabular}
\caption{\ATUA's state abstraction functions. Blue highlights the reducers introduced in finer granularity levels.}
\label{table:refinement}
\end{table}%


==> tables/budgets.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{7mm}|p{1.2cm}|p{10.5cm}|}
\hline

\textbf{Phase}&\textbf{Budget}&\textbf{Strategy}\\
\hline
\multirow{2}{*}{Phase1}&Phase&Infinite, i.e., all the target windows are exercised till stagnation is detected or all the targets are covered.\\
\cline{2-3}
&Reachability&Infinite, i.e., all the paths are traversed in this phase.\\
\cline{2-3}
 &Target&Infinite, i.e., all the target Inputs are tried in this phase.\\
\cline{2-3} 
  &Random Exploration&Set to $\mathit{scaleFactor}*\mathit{NumberOfActionsForActiveWindow}$. In our experiments, we set $\mathit{scaleFactor}$ to $1$ for an overall test budget of one hour, to $2$ for a test budget of five hours. Random exploration is triggered by either \emph{reachTargetNode} or \emph{identifyPathToTarget}.\\
 \hline 
 \multirow{3}{*}{Phase2}&Phase&Set to $\mathit{scaleFactor}*\mathit{NumberOfTargetWindows}$.\\
  \cline{2-3}
& Reachability&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. The value is reset every time a new TargetWindow is identified.  We set $\mathit{actionsThreshold}$ to $25$.\\
 \cline{2-3}
 & Target&Set to be equal to what remains of the {ReachabilityBudget} after the target window is reached. In other words, $\mathit{ReachabilityBudget} + \mathit{TargetBudget} = \mathit{scaleFactor}*\mathit{actionsThreshold}$ \\
  \cline{2-3}
 &Random Exploration&Set to $\mathit{scaleFactor}*\mathit{randomThreshold}$. Random exploration is triggered by either \emph{reachTargetNode} or \emph{identifyPathToTarget}. We set $\mathit{randomThreshold}$ equal to $\mathit{actionsThreshold}$.\\
\hline
 \multirow{3}{*}{Phase3}&Reachability&Not used in this phase.\\
 \cline{2-3}
 & Target&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. It is reset every time a new TargetEvent is identified.\\
 \cline{2-3}
&Random Exploration&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. Random exploration is triggered (1) to explore the related Window, (2) when the related Window cannot be reached through the identified path, (3) 
when the target Window cannot be reached through the identified path (see Section~\ref{sec:phase3}). We set $\mathit{randomThreshold}$ to $5$.\\
% \cline{2-3}
% & Target&.\\
\hline
\end{tabular}
\caption{Strategies adopted, in different \APPR phases, to define the budget allocated to distinct test activities.}
\label{table:budgets}
\end{table}%


==> tables/caseStudies_size.tex <==
\begin{table}[]
\caption{Apk size for each App version.}
\scriptsize
\begin{tabular}{|l|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{App}} & \multicolumn{1}{c|}{\textbf{Version}} & \multicolumn{1}{c|}{\textbf{Apk Size (MB)}} & \multicolumn{1}{c|}{\textbf{App Activities}} \\ \hline
\multirow{9}{*}{AD}                & 105                                   & 2.4                                         & 7                                            \\ \cline{2-4} 
                                   & 111                                   & 2.5                                         & 7                                            \\ \cline{2-4} 
                                   & 115                                   & 2.5                                         & 7                                            \\ \cline{2-4} 
                                   & 118                                   & 2.6                                         & 7                                            \\ \cline{2-4} 
                                   & 122                                   & 2.6                                         & 8                                            \\ \cline{2-4} 
                                   & 125                                   & 2.7                                         & 8                                            \\ \cline{2-4} 
                                   & 130                                   & 3.3                                         & 10                                           \\ \cline{2-4} 
                                   & 131                                   & 3.3                                         & 10                                           \\ \cline{2-4} 
                                   & 134                                   & 3.6                                         & 11                                           \\ \hline
\multirow{10}{*}{BM}               & 5.1.0                                 & 11.7                                        & 18                                           \\ \cline{2-4} 
                                   & 5.10.0                                & 16.4                                        & 14                                           \\ \cline{2-4} 
                                   & 5.11.0                                & 16.5                                        & 14                                           \\ \cline{2-4} 
                                   & 5.12.0                                & 17.2                                        & 14                                           \\ \cline{2-4} 
                                   & 5.13.0                                & 17.3                                        & 15                                           \\ \cline{2-4} 
                                   & 5.4.0                                 & 11.8                                        & 15                                           \\ \cline{2-4} 
                                   & 5.5.0                                 & 14.6                                        & 15                                           \\ \cline{2-4} 
                                   & 5.6.0                                 & 14.9                                        & 17                                           \\ \cline{2-4} 
                                   & 5.8.1                                 & 15.8                                        & 16                                           \\ \cline{2-4} 
                                   & 5.9.0                                 & 16                                          & 14                                           \\ \hline
\multirow{10}{*}{CM}               & 9.1                                   & 19.3                                        & 64                                           \\ \cline{2-4} 
                                   & 9.2                                   & 18.7                                        & 64                                           \\ \cline{2-4} 
                                   & 9.3                                   & 18.3                                        & 64                                           \\ \cline{2-4} 
                                   & 9.4                                   & 18.2                                        & 60                                           \\ \cline{2-4} 
                                   & 9.5                                   & 18.3                                        & 60                                           \\ \cline{2-4} 
                                   & 9.6                                   & 20.3                                        & 60                                           \\ \cline{2-4} 
                                   & 9.7                                   & 20.4                                        & 61                                           \\ \cline{2-4} 
                                   & 9.8                                   & 20.5                                        & 61                                           \\ \cline{2-4} 
                                   & 9.9                                   & 19.3                                        & 61                                           \\ \cline{2-4} 
                                   & 10                                    & 22.2                                        & 61                                           \\ \hline
\multirow{5}{*}{FM}                & 44                                    & 5.4                                         & 7                                            \\ \cline{2-4} 
                                   & 53                                    & 6                                           & 7                                            \\ \cline{2-4} 
                                   & 77                                    & 8                                           & 9                                            \\ \cline{2-4} 
                                   & 79                                    & 8                                           & 9                                            \\ \cline{2-4} 
                                   & 82                                    & 8.4                                         & 9                                            \\ \hline
\multirow{5}{*}{WI}                & 198                                   & 20                                          & 24                                           \\ \cline{2-4} 
                                   & 10239                                 & 10.3                                        & 31                                           \\ \cline{2-4} 
                                   & 10263                                 & 10.7                                        & 33                                           \\ \cline{2-4} 
                                   & 10264                                 & 10.7                                        & 33                                           \\ \cline{2-4} 
                                   & 10269                                 & 10.4                                        & 33                                           \\ \hline
\multirow{9}{*}{VP}                & 3.1.4                                 & 28.3                                        & 28                                           \\ \cline{2-4} 
                                   & 3.1.5                                 & 28.3                                        & 28                                           \\ \cline{2-4} 
                                   & 3.1.7                                 & 28.3                                        & 28                                           \\ \cline{2-4} 
                                   & 3.2.12                                & 28.6                                        & 33                                           \\ \cline{2-4} 
                                   & 3.2.2                                 & 28.2                                        & 33                                           \\ \cline{2-4} 
                                   & 3.2.3                                 & 28.3                                        & 33                                           \\ \cline{2-4} 
                                   & 3.2.6                                 & 28.3                                        & 33                                           \\ \cline{2-4} 
                                   & 3.2.7                                 & 28.3                                        & 33                                           \\ \cline{2-4} 
                                   & 3.2.9                                 & 28.3                                        & 33                                           \\ \hline
\multirow{10}{*}{YM}               & 1.16.0                                & 25.6                                        & 23                                           \\ \cline{2-4} 
                                   & 1.16.1                                & 25.6                                        & 23                                           \\ \cline{2-4} 
                                   & 1.16.2.                               & 25.7                                        & 24                                           \\ \cline{2-4} 
                                   & 1.17.3                                & 25.2                                        & 24                                           \\ \cline{2-4} 
                                   & 1.18.1                                & 26.1                                        & 24                                           \\ \cline{2-4} 
                                   & 1.19.1                                & 24.9                                        & 24                                           \\ \cline{2-4} 
                                   & 1.20.1                                & 25.8                                        & 24                                           \\ \cline{2-4} 
                                   & 1.20.3                                & 30.7                                        & 24                                           \\ \cline{2-4} 
                                   & 1.20.5                                & 32.3                                        & 24                                           \\ \cline{2-4} 
                                   & 1.20.7                                & 32.3                                        & 25                                           \\ \hline
\end{tabular}
\end{table}

==> tables/effectSizeInputs.tex <==
%% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for Figure~\ref{fig:RQ3:Inputs:1} and ~\ref{fig:RQ3:Inputs:5}.}
\label{table:effectSize:inputs}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{S}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
1&<0.05&<0.05&<0.05&.018&.000&.000&<0.05&<0.05&<0.05&\R{.630}&.000&.000\\
2&<0.05&<0.05&<0.05&.000&.000&.000&<0.05&<0.05&<0.05&.020&.000&.000\\
3&<0.05&<0.05&<0.05&.039&.000&.000&<0.05&<0.05&<0.05&.093&.000&.000\\
4&<0.05&<0.05&<0.05&.099&.000&.000&<0.05&<0.05&<0.05&.278&.000&.000\\
5&<0.05&<0.05&<0.05&.074&.000&.397&<0.05&<0.05&\R{0.81}&.090&.000&\R{.490}\\
6&<0.05&<0.05&<0.05&.360&.000&.000&\R{0.15}&<0.05&<0.05&.425&.000&.000\\
7&<0.05&<0.05&<0.05&.117&.000&.000&<0.05&<0.05&<0.05&.123&.000&.000\\
8&<0.05&<0.05&<0.05&.405&.000&.000&<0.05&<0.05&<0.05&.075&.000&.000\\
9&<0.05&<0.05&<0.05&\R{.048}&.000&.000&<0.05&<0.05&<0.05&.001&.000&.000\\
\hline
\end{tabular}

\textbf{Legend}: \emph{S}, subject. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$) or no higher chances of generating less instructions ($A_{12} > 0.44$) than state-of-the-art approaches.
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/effectSizeInputsRatio.tex <==
%% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for target instructions/inputs ratios.}
\label{table:effectSize:ratio}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{S}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
1&\R{0.10}&<0.05&<0.05&.728&1.00&.975&\R{0.69}&<0.05&<0.05&\R{.555}&.963&.901\\
2&\R{0.17}&<0.05&<0.05&.703&.906&.875&\R{0.14}&<0.05&<0.05&.719&.938&.875\\
3&\R{0.29}&\R{0.09}&\R{0.09}&.700&.820&.820&\R{0.25}&\R{0.08}&\R{0.17}&.720&.840&.760\\
4&\R{0.33}&<0.05&\R{0.05}&.636&.895&.772&\R{0.38}&<0.05&<0.05&.623&.895&.747\\
5&\R{0.17}&<0.05&<0.05&.691&1.00&.901&\R{0.17}&<0.05&<0.05&.691&.950&.827\\
6&\R{0.63}&<0.05&<0.05&.583&1.00&1.00&\R{0.52}&<0.05&<0.05&.611&1.00&1.00\\
7&\R{0.27}&<0.05&<0.05&.654&1.00&1.00&\R{0.27}&<0.05&<0.05&.654&1.00&1.00\\
8&\R{0.60}&<0.05&<0.05&.578&1.00&.953&\R{0.92}&<0.05&<0.05&\R{.516}&.968&.906\\
9&\R{0.39}&<0.05&<0.05&.642&1.00&1.00&<0.05&<0.05&<0.05&.914&1.00&1.00
\\
\hline
\end{tabular}

\textbf{Legend}: \emph{S}, subject. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$) or no higher likelihood of achieving a higher instructions/inputs ratio (i.e., $A_{12} < 0.56$) than state-of-the-art approaches.
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/effectSizeRQ21.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for RQ2.}
\label{table:effectSize:rq21}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{C}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
&
\multicolumn{12}{c|}{\textbf{Coverage of target methods}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.857&.994&.956&<0.05&<0.05&\R{0.14}&.703&.935&.564\\
2&<0.05&<0.05&<0.05&.733&.868&.703&<0.05&<0.05&<0.05&.774&.832&.623\\
3&\R{0.41}&<0.05&<0.05&\R{.548}&.795&.684&\R{0.61}&<0.05&0.99&\R{.529}&.767&\R{.501}\\
4&\R{0.16}&<0.05&\R{0.07}&.560&.852&.577&\R{0.16}&<0.05&\R{0.08}&.560&.760&.575\\
5&<0.05&<0.05&<0.05&.735&.814&.920&<0.05&<0.05&<0.05&.713&.702&.841\\
6&\R{0.08}&<0.05&<0.05&.587&.838&.689&\R{0.2}&<0.05&<0.05&.564&.719&.681\\
7&<0.05&<0.05&<0.05&.614&.836&.762&\R{0.78}&<0.05&<0.05&\R{.488}&.879&.879\\
8&\R{0.23}&<0.05&<0.05&\R{.554}&.997&.972&\R{0.05}&<0.05&<0.05&.588&.995&.892\\
9&<0.05&<0.05&<0.05&.587&.981&.878&<0.05&<0.05&<0.05&.685&.992&.918\\
\hline
&\multicolumn{12}{c|}{\textbf{Coverage of target instructions}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.853&.991&.936&<0.05&<0.05&\R{0.15}&.735&.884&.562\\
2&<0.05&<0.05&<0.05&.707&.843&.783&<0.05&<0.05&<0.05&.756&.829&.721\\
3&\R{0.31}&<0.05&\R{0.14}&\R{.559}&.774&.585&\R{0.18}&<0.05&\R{0.70}&.577&.705&\R{.478}\\
4&<0.05&<0.05&\R{0.07}&.600&.861&.579&\R{0.05}&<0.05&<0.05&.584&.764&.594\\
5&<0.05&<0.05&<0.05&.684&.748&.886&<0.05&<0.05&<0.05&.659&.623&.822\\
6&\R{0.42}&<0.05&<0.05&\R{.542}&.788&.827&\R{0.47}&<0.05&<0.05&\R{.538}&.727&.786\\
7&<0.05&<0.05&<0.05&.598&.735&.695&\R{0.65}&<0.05&<0.05&\R{.480}&.780&.780\\
8&\R{0.06}&<0.05&<0.05&.586&.999&.984&\R{0.33}&<0.05&<0.05&.633&.999&.936\\
9&0.05&<0.05&<0.05&.584&.980&.822&<0.05&<0.05&<0.05&.671&.988&.896\\
\hline
\end{tabular}

\textbf{Legend}: \emph{C}, case study. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$ ) or no higher likelihood (i.e., $A_{12} < 0.56$) of covering more targets  than state-of-the-art approaches.
\end{table}%


==> tables/effectSizeRQ22.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for RQ2.2.}
\label{table:effectSize:rq22}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
}
\hline
\textbf{}&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{C}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
&
\multicolumn{12}{c|}{\textbf{Coverage of target methods}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.890&1.00&.890
&<0.05&<0.05&<0.05&.640&.820&\R{.320}\\
2&<0.05&<0.05&<0.05&\R{.370}&.990&.850
&<0.05&<0.05&<0.05&.890&1.00&1.00\\
3&\R{0.80}&<0.05&<0.05&\R{.350}&1.00&.900
&\R{0.46}&<0.05&0.99&.845&.975&.600\\
4&<0.05&<0.05&<0.05&.960&1.00&.950
&<0.05&<0.05&<0.05&.950&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.650&1.00&.920&
<0.05&<0.05&<0.05&.690&1.00&.630\\
7&<0.05&<0.05&<0.05&.950&1.00&.970
&<0.05&<0.05&<0.05&\R{.530}&1.00&1.00\\
8&\R{0.46}&<0.05&<0.05&\R{.530}&1.00&.990
&<0.05&<0.05&<0.05&.810&1.00&1.00\\
9&<0.05&<0.05&\R{1.00}&.650&1.00&1.00
&<0.05&<0.05&\R{1.00}&.800&1.00&1.00\\
\hline
&\multicolumn{12}{c|}{\textbf{Coverage of target instructions}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.900&.990&.880
&<0.05&<0.05&<0.05&.660&.760&\R{.350}\\
2&<0.05&<0.05&<0.05&.620&.980&.560
&<0.05&<0.05&<0.05&.940&.980&\R{.200}\\
3&\R{0.81}&<0.05&<0.05&\R{.490}&1.00&.980
&<0.05&<0.05&<0.05&.960&1.00&.760\\
4&<0.05&<0.05&<0.05&.950&1.00&.940
&<0.05&<0.05&<0.05&.940&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.790&1.00&.610
&<0.05&<0.05&<0.05&.720&1.00&\R{.400}\\
7&<0.05&<0.05&<0.05&.970&1.00&.990
&<0.05&<0.05&<0.05&\R{.550}&1.00&1.00\\
8&<0.05&<0.05&<0.05&.660&1.00&.990
&<0.05&<0.05&<0.05&.900&1.00&1.00\\
9&\R{0.05}&<0.05&\R{1.00}&.680&1.00&.728
&<0.05&<0.05&\R{1.00}&.810&1.00&.656\\
\hline
\end{tabular}
\textbf{Legend}: \emph{C}, case study. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$ ) or no higher likelihood (i.e., $A_{12} < 0.56$) of covering more targets  than state-of-the-art approaches.
\end{table}%


==> tables/ewtgmodel.tex <==
% \begin{table*}
% \footnotesize
% \begin{tabular}{ |p{2cm}|p{1.5cm}|p{2cm}|p{9cm}|  }
%  \hline
%  \textbf{EWTG Element} & \textbf{Type} & \textbf{Attribute / Reference name} &
%  \textbf{Description}\\
%  \hline
%  \multirow{4}{*}{Window}   & Attribute & className & for Activity and Dialog, this is the name of implementation class; for OptionsMenu and ContextMenu, this is the className of the Activity declaring the menu.\\
%  \cline{2-4}
%   & Attribute & windowType & i.e., Activity, Dialog, OptionsMenu, ContextMenu. \\
%  \cline{2-4}
% & Reference & ownerActivity & reserved only for Dialog; this is the Activity that use the dialog.\\
%  \cline{2-4}
%  & Attribute & createdLocation & reserved only for Dialog; this is the statement (instruction) where the dialog is instantiated. \\
%  \hline
%  \multirow{4}{*}{Widget}  & Attribute & className & the class name of Widget's type (e.g. LinearLayout, TextView). \\
%  \cline{2-4}
%  & Attribute & resourceId & the id name assigned to the Widget in an xml layout. \\
%  \cline{2-4}
%  & Reference& parent & the containing widget \\
%  \cline{2-4}
%  & Attribute& xpath & the XMLPath of the widget, which helps to locate the widget in a GUI tree. \\
%  \hline
%  \multirow{4}{*}{Transition} & Attribute& action & e.g. click, swipe, press back. \\
%  \cline{2-4}
%  &Attribute &targetWidget & the widget trigger with the action. Some actions do not need a target (e.g. press back, press menu.)\\
%  \cline{2-4}
%  &Reference &source & the window before executing the transition\\
%  \cline{2-4}
%  &Reference& destination & the window after executing the transition\\
%  \hline
% \end{tabular}
% \caption{EWTG elements considered when deriving an RCVDiff model to compare EWTGs belonging to two App versions}
% \label{tab:ewtgmodel}
% \end{table*}

\begin{table}
\footnotesize
\begin{tabular}{ |p{2.7cm}|p{1cm}|p{4cm}|  }
 \hline
 \textbf{EWTG Element} & \textbf{RCVDiff Element} & \textbf{Description}\\
 \hline
 Window instance  & MElement& A Window.\\
 className attribute  & MAttribute& implementng class or className declaring the menu (for menus)\\
  windowType attribute & MAttribute&Activity, Dialog, OptionsMenu, or ContextMenu\\
 ownerActivity association & MReference& Activity that uses the Window, if a Window is a Dialog.\\
 createdLocation attribute & MAttribute & Statement instantiating the dialog. \\
 \hline
 Widget instance  & MElement& A Widget.\\
 className attribute & MAttribute &  Widget's type (e.g. LinearLayout). \\
 resourceId attribute & MAttribute & ID assigned to the Widget in a layout. \\
 parent attribute & MReference&  Containing Widget. \\
 xpath attribute & MAttribute&  XMLPath of the widget. \\
 \hline
 Transition instance  & MElement& A Transition.\\
 action attribute & MAttribute& Action (e.g., click, swipe, press back). \\
 targetWidget attribute & MAttribute & The target of the corresponding Action.\\
 source attribute &MReference & Active Window before the Transition.\\
 destination attribute& MReference& Active Window after the Transition.\\
 \hline
\end{tabular}
\caption{EWTG elements considered when deriving an RCVDiff model to compare EWTGs belonging to two App versions}
\label{tab:ewtgmodel}
\end{table}

==> tables/exerciseStrategies.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{2cm}|p{11cm}|}
\hline

\textbf{Widget type}&\textbf{Input generation procedure}\\
\hline
Any widget& Trigger an InputEvent among the ones for which an event handler has been declared.\\
\hline
Textarea & Randomly apply one of the following: 
(1) leave it empty,
(2) reuse a string already used in the past,
(3) reuse a string already used for the same widget,
(4) reuse a string literal extracted with static analysis,
(5) use a randomly generated alphabetic string~\cite{Borges-Droidmate2-ASE-2018},
(6) use a randomly generated non alphabetic char.\\
\hline
Radio buttons and check boxes& Randomly select one of the possible options (e.g., checked/not checked, for check boxes). \\
\hline
Widgets with manual input& Randomly select one of the available InputInstances, if more than one is available, and then assign the specified value.\\
\hline
Intent& If the current activity declares an Intent, it triggers the Intent specified by the engineer.\\
\hline
\end{tabular}
\caption{\APPR Input generation procedures.}
\label{table:exerciseWidgets}
\end{table}%


==> tables/fap.tex <==
% !TEX root =  ../MAIN.tex

\begin{figure}[htp]
\footnotesize
\begin{tabular}{|p{0.5cm}|p{7.5cm}|}
\hline
$w_1=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\} \rangle$\\
$w_2=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\}, \{i=1,t=LL,a=\emptyset\}  \rangle$\\
$w_3=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\}, \{i=2,t=LL,a=\emptyset\}, \{i=1,t=LL,a=\mathit{Radio}\}  \rangle$\\
\hline
\end{tabular}
FL: FrameLayout, LL=LinearLayout, LV=ListView, TW=TextView.

\caption{Full Attribute Paths for the widgets in Figure~\ref{}.}
\label{fig:fullAttributePaths}
\end{figure}%


==> tables/manualInputs.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Case studies with manual inputs.}
\label{table:manualInputs}
\begin{tabular}{
|@{\hspace{1pt}}p{1.5cm}@{\hspace{1pt}}|
p{6cm}|
p{1cm}|
p{1cm}|
p{1cm}|
}
\hline
\textbf{Case study}&
\textbf{Feature tested}&
\multicolumn{1}{c|}{\textbf{\# Windows}}&
\multicolumn{1}{c|}{\textbf{\# Data fields}}&
\multicolumn{1}{c|}{\textbf{\# Instances}}\\
\hline
\multirow{2}{*}{Wikipedia}&
Log-in functionality&1&2&1\\
\cline{2-5}
&Creation of a new account&
1&
4&
14								
\\
\hline
\multirow{2}{*}{VLC}
&
Play a video stream using a URL
&
1
&
1
&
2
\\
\cline{2-5}
&
Populate the library with all the videos on the device
&
1
&
1
&
1
\\
\hline
Nuzzel
&
Request an e-mail newsletter
&
1
&
1
&
1
\\
\hline
\end{tabular}
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/tableSignatures.tex <==
\begin{table}[]
\begin{tabular}{ |c|c|c| } 
 \hline
 \textbf{EWTG Element} & \textbf{Attribute/Reference} &
 \textbf{Description}\\
 \hline
 Window & className & \\
 \hline
  & windowType & \\
 \hline
& ownerActivity & \\
 \hline
 & createdLocation & \\
\end{tabular}
\caption{Signatures of different types of element}
\label{tab:signature}
\end{table}

==> tables/utaCountBySubject.tex <==
\begin{table}[]
    \centering
    \caption{Statistics (Max, Min and Average) for the number of UTAs exercised for each App version tested by \APPR}
    \label{tab:rq1_statistics_numberUtas}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|}
    \hline
App&Version&$\mathrm{UTA_{max}}$&$\mathrm UTA_{min}$&$\mathrm UTA_{avg}$\\ \hline
activitydiary&V1&11&6&9.0\\
activitydiary&V2&4&3&3.1\\
activitydiary&V3&15&12&13.5\\
activitydiary&V4&72&57&64.1\\
activitydiary&V5&37&30&33.1\\
activitydiary&V6&41&26&31.8\\
activitydiary&V7&1&1&1.0\\
activitydiary&V8&54&42&47.8\\
amazefile&V1&100&69&83.0\\
amazefile&V2&78&65&71.5\\
amazefile&V3&6&4&5.1\\
amazefile&V4&153&110&123.3\\
bbc&V1&38&23&28.8\\
bbc&V2&6&3&4.5\\
bbc&V3&10&9&9.3\\
bbc&V4&8&7&7.6\\
bbc&V5&40&34&37.3\\
bbc&V6&39&32&36.4\\
bbc&V7&56&48&51.3\\
bbc&V8&12&8&10.1\\
bbc&V9&14&10&12.0\\
citymapper&V1&25&17&20.7\\
citymapper&V2&20&16&18.0\\
citymapper&V3&24&13&16.5\\
citymapper&V4&30&21&25.5\\
citymapper&V5&46&30&38.4\\
citymapper&V6&32&23&27.1\\
citymapper&V7&33&22&27.3\\
citymapper&V8&8&4&5.9\\
citymapper&V9&22&15&19.6\\
vlc&V1&239&163&198.0\\
vlc&V2&28&19&24.5\\
vlc&V3&308&197&256.1\\
vlc&V4&93&65&76.5\\
vlc&V5&11&9&10.0\\
vlc&V6&43&28&36.4\\
vlc&V7&36&27&31.7\\
vlc&V8&40&29&32.3\\
wikipedia&V1&56&48&51.6\\
wikipedia&V2&216&179&197.8\\
wikipedia&V3&135&102&116.2\\
wikipedia&V4&10&8&8.8\\
wikipedia&V5&47&36&43.0\\
yahooweather&V1&7&5&6.1\\
yahooweather&V2&4&2&3.7\\
yahooweather&V3&85&64&73.6\\
yahooweather&V4&13&11&12.1\\
yahooweather&V5&15&12&13.0\\
yahooweather&V6&43&15&35.8\\
yahooweather&V7&47&34&40.3\\
yahooweather&V8&11&6&7.4\\
yahooweather&V9&7&5&6.4\\ \hline
    \end{tabular}

\end{table}
